DeepPerform: An Efficient Approach for Performance Testing of Resource-Constrained Neural Networks

Today, an increasing number of Adaptive Deep Neural Networks (AdNNs) are being used on resource-constrained embedded devices. We observe that, similar to traditional software, redundant computation exists in AdNNs, resulting in considerable performance degradation. The performance degradation is dependent on the input and is referred to as input-dependent performance bottlenecks (IDPBs). To ensure an AdNN satisfies the performance requirements of resource-constrained applications, it is essential to conduct performance testing to detect IDPBs in the AdNN. Existing neural network testing methods are primarily concerned with correctness testing, which does not involve performance testing. To fill this gap, we propose DeepPerform, a scalable approach to generate test samples to detect the IDPBs in AdNNs. We first demonstrate how the problem of generating performance test samples detecting IDPBs can be formulated as an optimization problem. Following that, we demonstrate how DeepPerform efficiently handles the optimization problem by learning and estimating the distribution of AdNNs' computational consumption. We evaluate DeepPerform on three widely used datasets against five popular AdNN models. The results show that DeepPerform generates test samples that cause more severe performance degradation (FLOPs: increase up to 552\%). Furthermore, DeepPerform is substantially more efficient than the baseline methods in generating test inputs(runtime overhead: only 6-10 milliseconds).

==> Evaluation/config.tex <==
\subsection{Configuration Sensitivity}
\label{sec:config}


As discussed in \secref{sec:background}, AdNNs require configuring the threshold $\tau_i$ to allocate computational resources. In this section, we evaluate whether the test samples generated from \tool could degrade the AdNNs' performance under different system configuration.
We configure $\tau_i = 0.3, 0.4, 0.5, 0.6, 0.7$ and measure the maximum FLOPs increments. 
Notice that we train \tool only with $\tau_i=0.5$ and test the performance degradation with different $\tau_i$.
The maximum FLOPs increment ratio under different system configurations are listed in \tabref{tab:configure}.
For all experimental settings, the maximum FLOPs increment ratio keeps a stable value~(\eg 79.19-90.48, 233.33-250.00, 600.00-800.00).
The results imply that the test samples generated by \tool can increase the computational complexity under different configurations, and the maximum increment ratio is stable as the configuration changes. 




\input{table/config}



\noindent
\\
\fbox{%
  \parbox{0.475\textwidth}{%
       Therefore, we answer RQ4 as follows: \textit{The test samples generated by \tool will increase the computational complexity under different configurations.}}
}\\[0.1pt]

==> Evaluation/hardware.tex <==
\subsection{Hardware Platform Sensitivity}
\label{sec:hardware}

In this section, we evaluate whether the test samples generated from \tool could still degrade the system performance on different hardware platforms.


We select four popular hardware platforms, 

==> Evaluation/sensitivity_1.tex <==

\subsection{Sensitivity}
\label{sec:sensitive}

In this section, we conduct two experiments to show that \tool can generate effective test samples under different settings.

\noindent\textbf{Configuration Sensitivity.} As discussed in \secref{sec:background}, AdNNs require configuring the threshold $\tau_i$ to set the accuracy-performance tradeoff mode. In this section, we evaluate whether the test samples generated from \tool could degrade the AdNNs' performance under different modes.
Specifically, we set the threshold $\tau_i$ in \equref{eq:new2} and \equref{eq:new3} as $0.3, 0.4, 0.5, 0.6, 0.7$ and measure the maximum FLOPs increments. 
Notice that we train \tool with $\tau_i=0.5$ and test the performance degradation with different $\tau_i$.
The maximum FLOPs increment ratio under different system configurations are listed in \tabref{tab:configure}.
For all experimental settings, the maximum FLOPs increment ratio keeps a stable value~(\eg 79.17-82.91, 175.59-250.00).
The results imply that the test samples generated by \tool can increase the computational complexity under different configurations, and the maximum FLOPs increment ratio is stable as the configuration changes. 




\input{LaTeX/table/config}



\noindent\textbf{Hardware Sensitivity.} We next evaluate the effectiveness of our approach on different hardware platforms. In particular, we select Intel Xeon E5-2660 V3 CPU and Nvidia 1080 Ti as our experimental hardware platforms and measure the maximum performance degradation ratio on those selected platforms. The test samples generated by \tool, as shown in \tabref{tab:hardware},  cause severe and stable runtime performance degradation on different hardware platforms. As a result, we conclude that \tool is not sensitive to hardware platforms.



\input{LaTeX/table/hardware}


\vspace{-5mm}
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=8cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
Answers to \textbf{RQ4}:  \textit{\tool is not sensitive to AdNNs' configurations, and hardware platforms.}
\end{tcolorbox}
\end{center}



==> table/effective_l2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{@{}c|l|l|l|l|l|llll|l|l|l|l@{}}
\toprule
\multirow{3}{*}{\textbf{Device}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Subject}}} & \multicolumn{4}{c|}{\textbf{I-FLOPs}}                                                     & \multicolumn{4}{c}{\textbf{I-Latency}}                                                                 & \multicolumn{4}{c|}{\textbf{I-Energy}}                                                    \\ \cmidrule(l){3-14} 
                                 & \multicolumn{1}{c|}{}                                  & \multicolumn{2}{c|}{\textbf{mean}}          & \multicolumn{2}{c|}{\textbf{max}}           & \multicolumn{2}{c|}{\textbf{mean}}                       & \multicolumn{2}{c|}{\textbf{max}}           & \multicolumn{2}{c|}{\textbf{mean}}          & \multicolumn{2}{c|}{\textbf{max}}           \\ \cmidrule(l){3-14} 
                                 & \multicolumn{1}{c|}{}                                  & \multicolumn{2}{c|}{\textbf{baseline/ours}} & \multicolumn{2}{c|}{\textbf{baseline/ours}} & \multicolumn{2}{c|}{\textbf{baseline/ours}}              & \multicolumn{2}{c|}{\textbf{baseline/ours}} & \multicolumn{2}{c|}{\textbf{baseline/ours}} & \multicolumn{2}{c|}{\textbf{baseline/ours}} \\ \midrule
\multirow{5}{*}{\textbf{CPU}}    & \textbf{SkipNet\_CIFAR10}                              & 9.55                   & 32.24              & 18.43                & 77.26                & \multicolumn{1}{l|}{30.20} & \multicolumn{1}{l|}{25.83}  & \multicolumn{1}{l|}{69.39}      & 52.89     & 3.28                 & 26.23                & 13.22                & 53.18                \\ \cmidrule(l){2-14} 
                                 & \textbf{BlockDrop\_CIFAR10}                            & 13.67                  & 19.24              & 162.58               & 175.59               & \multicolumn{1}{l|}{12.39} & \multicolumn{1}{l|}{22.91}  & \multicolumn{1}{l|}{143.85}     & 144.02    & 12.73                & 23.60                & 148.19               & 150.08               \\ \cmidrule(l){2-14} 
                                 & \textbf{RANet\_CIFAR100}                               & 5.92                   & 51.47              & 218.73               & 283.33               & \multicolumn{1}{l|}{34.94} & \multicolumn{1}{l|}{66.15}  & \multicolumn{1}{l|}{370.23}     & 503.52    & 35.07                & 68.17                & 387.07               & 518.69               \\ \cmidrule(l){2-14} 
                                 & \textbf{DeepShallow\_CIFAR100}                         & -19.08                 & -2.53              & 380.67               & 287.98               & \multicolumn{1}{l|}{26.46} & \multicolumn{1}{l|}{-9.73}  & \multicolumn{1}{l|}{601.46}     & 244.96    & 25.43                & 8.73                 & 666.08               & 252.58               \\ \cmidrule(l){2-14} 
                                 & \textbf{DeepShallow\_SVHN}                             & 17.03                  & 60.25              & 498.29               & 498.29               & \multicolumn{1}{l|}{29.67} & \multicolumn{1}{l|}{168.16} & \multicolumn{1}{l|}{1371.23}    & 1665.16   & 31.31                & 172.64               & 1372.83              & 1646.98              \\ \midrule
\multirow{5}{*}{\textbf{GPU}}    & \textbf{SkipNet\_CIFAR10}                              & 9.55                   & 32.24              & 18.43                & 77.26                & \multicolumn{1}{l|}{1.91}  & \multicolumn{1}{l|}{4.94}   & \multicolumn{1}{l|}{24.46}      & 23.28     & 1.90                 & 4.94                 & 16.79                & 18.43                \\ \cmidrule(l){2-14} 
                                 & \textbf{BlockDrop\_CIFAR10}                            & 13.67                  & 19.24              & 162.58               & 175.59               & \multicolumn{1}{l|}{3.20}  & \multicolumn{1}{l|}{5.58}   & \multicolumn{1}{l|}{39.88}      & 47.95     & 4.48                 & 6.08                 & 46.45                & 50.96                \\ \cmidrule(l){2-14} 
                                 & \textbf{RANet\_CIFAR100}                               & 5.92                   & 51.47              & 218.73               & 283.33               & \multicolumn{1}{l|}{51.53} & \multicolumn{1}{l|}{62.86}  & \multicolumn{1}{l|}{454.77}     & 615.77    & 56.43                & 77.46                & 557.93               & 769.88               \\ \cmidrule(l){2-14} 
                                 & \textbf{DeepShallow\_CIFAR100}                         & -19.08                 & -2.53              & 380.67               & 287.98               & \multicolumn{1}{l|}{42.85} & \multicolumn{1}{l|}{-10.88} & \multicolumn{1}{l|}{514.67}     & 219.86    & 34.29                & -13.85               & 531.57               & 292.78               \\ \cmidrule(l){2-14} 
                                 & \textbf{DeepShallow\_SVHN}                             & 17.03                  & 60.25              & 498.29               & 498.29               & \multicolumn{1}{l|}{9.21}  & \multicolumn{1}{l|}{37.94}  & \multicolumn{1}{l|}{280.00}     & 321.70    & 15.41                & 63.16                & 348.33               & 462.38               \\ \bottomrule
\end{tabular}
\end{table*}

==> table/effective_linf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{@{}clcccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Device}}                   & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{Subject}}} & \multicolumn{4}{c}{\textbf{I-FLOPs}}                                                                                & \multicolumn{4}{c}{\textbf{I-Latency}}                                                                                  & \multicolumn{4}{c}{\textbf{I-Energy}}                                                                   \\ \cmidrule(l){3-14} 
                                                   & \multicolumn{1}{c}{}                                  & \multicolumn{2}{c|}{\textbf{mean}}                      & \multicolumn{2}{c|}{\textbf{max}}                         & \multicolumn{2}{c|}{\textbf{mean}}                        & \multicolumn{2}{c|}{\textbf{max}}                           & \multicolumn{2}{c|}{\textbf{mean}}                        & \multicolumn{2}{c|}{\textbf{max}}           \\ \cmidrule(l){3-14} 
                                                   & \multicolumn{1}{c}{}                                  & \multicolumn{2}{c|}{\textbf{baseline/ours}}             & \multicolumn{2}{c|}{\textbf{baseline/ours}}               & \multicolumn{2}{c|}{\textbf{baseline/ours}}               & \multicolumn{2}{c|}{\textbf{baseline/ours}}                 & \multicolumn{2}{c|}{\textbf{baseline/ours}}               & \multicolumn{2}{c|}{\textbf{baseline/ours}} \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{CPU}}} & \multicolumn{1}{l|}{\textbf{SkipNet\_CIFAR10}}        & \multicolumn{1}{c|}{18.12} & \multicolumn{1}{c|}{29.50} & \multicolumn{1}{c|}{43.82}  & \multicolumn{1}{c|}{72.43}  & \multicolumn{1}{c|}{46.73}  & \multicolumn{1}{c|}{23.44}  & \multicolumn{1}{c|}{89.92}   & \multicolumn{1}{c|}{45.34}   & \multicolumn{1}{c|}{18.29}  & \multicolumn{1}{c|}{23.81}  & \multicolumn{1}{c|}{42.87}      & 46.34     \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{BlockDrop\_CIFAR10}}      & \multicolumn{1}{c|}{11.56} & \multicolumn{1}{c|}{13.40} & \multicolumn{1}{c|}{132.36} & \multicolumn{1}{c|}{175.59} & \multicolumn{1}{c|}{25.10}  & \multicolumn{1}{c|}{18.64}  & \multicolumn{1}{c|}{142.13}  & \multicolumn{1}{c|}{137.76}  & \multicolumn{1}{c|}{25.35}  & \multicolumn{1}{c|}{18.99}  & \multicolumn{1}{c|}{148.17}     & 139.72    \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{RANet\_CIFAR100}}         & \multicolumn{1}{c|}{10.53} & \multicolumn{1}{c|}{63.57} & \multicolumn{1}{c|}{498.99} & \multicolumn{1}{c|}{468.92} & \multicolumn{1}{c|}{58.37}  & \multicolumn{1}{c|}{81.47}  & \multicolumn{1}{c|}{1654.41} & \multicolumn{1}{c|}{840.61}  & \multicolumn{1}{c|}{58.40}  & \multicolumn{1}{c|}{84.30}  & \multicolumn{1}{c|}{1685.07}    & 874.13    \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{DeepShallow\_CIFAR100}}   & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{c|}{66.69} & \multicolumn{1}{c|}{552.00} & \multicolumn{1}{c|}{552.00} & \multicolumn{1}{c|}{122.24} & \multicolumn{1}{c|}{51.44}  & \multicolumn{1}{c|}{839.38}  & \multicolumn{1}{c|}{475.56}  & \multicolumn{1}{c|}{123.39} & \multicolumn{1}{c|}{55.49}  & \multicolumn{1}{c|}{845.35}     & 482.73    \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{DeepShallow\_SVHN}}       & \multicolumn{1}{c|}{37.75} & \multicolumn{1}{c|}{52.92} & \multicolumn{1}{c|}{289.83} & \multicolumn{1}{c|}{498.29} & \multicolumn{1}{c|}{11.15}  & \multicolumn{1}{c|}{106.30} & \multicolumn{1}{c|}{658.84}  & \multicolumn{1}{c|}{1265.54} & \multicolumn{1}{c|}{12.03}  & \multicolumn{1}{c|}{110.35} & \multicolumn{1}{c|}{673.28}     & 1256.89   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{GPU}}} & \multicolumn{1}{l|}{\textbf{SkipNet\_CIFAR10}}        & \multicolumn{1}{c|}{18.12} & \multicolumn{1}{c|}{29.50} & \multicolumn{1}{c|}{43.82}  & \multicolumn{1}{c|}{72.43}  & \multicolumn{1}{c|}{4.94}   & \multicolumn{1}{c|}{2.75}   & \multicolumn{1}{c|}{25.34}   & \multicolumn{1}{c|}{17.27}   & \multicolumn{1}{c|}{4.99}   & \multicolumn{1}{c|}{2.78}   & \multicolumn{1}{c|}{20.79}      & 17.68     \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{BlockDrop\_CIFAR10}}      & \multicolumn{1}{c|}{11.56} & \multicolumn{1}{c|}{13.40} & \multicolumn{1}{c|}{132.36} & \multicolumn{1}{c|}{175.59} & \multicolumn{1}{c|}{9.39}   & \multicolumn{1}{c|}{3.38}   & \multicolumn{1}{c|}{53.58}   & \multicolumn{1}{c|}{48.03}   & \multicolumn{1}{c|}{8.88}   & \multicolumn{1}{c|}{3.87}   & \multicolumn{1}{c|}{59.00}      & 49.40     \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{RANet\_CIFAR100}}         & \multicolumn{1}{c|}{10.53} & \multicolumn{1}{c|}{63.57} & \multicolumn{1}{c|}{498.99} & \multicolumn{1}{c|}{468.92} & \multicolumn{1}{c|}{84.31}  & \multicolumn{1}{c|}{86.70}  & \multicolumn{1}{c|}{1968.54} & \multicolumn{1}{c|}{1085.29} & \multicolumn{1}{c|}{91.48}  & \multicolumn{1}{c|}{113.92} & \multicolumn{1}{c|}{2446.52}    & 1332.11   \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \multicolumn{1}{l|}{\textbf{DeepShallow\_CIFAR100}}   & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{c|}{66.69} & \multicolumn{1}{c|}{552.00} & \multicolumn{1}{c|}{552.00} & \multicolumn{1}{c|}{103.01} & \multicolumn{1}{c|}{42.21}  & \multicolumn{1}{c|}{796.69}  & \multicolumn{1}{c|}{386.69}  & \multicolumn{1}{c|}{88.57}  & \multicolumn{1}{c|}{49.16}  & \multicolumn{1}{c|}{838.78}     & 467.48    \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                              & \textbf{DeepShallow\_SVHN}                            & 37.75                      & 52.92                      & 289.83                      & 498.29                      & 5.27                        & 33.27                       & 187.84                       & 314.62                       & 8.78                        & 51.35                       & 231.24                          & 392.15    \\ \bottomrule
\end{tabular}
\end{table*}

==> table/model.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Model accuracy and average blocks}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{CIFAR 10}} & \multicolumn{2}{c}{\textbf{CIFAR 100}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{}                                & \textbf{Acc}     & \textbf{Blocks}     & \textbf{Acc}     & \textbf{Blocks}     \\ \midrule
\textbf{BlockDrop}                                   & 93.55            & 16.93               & 73.66            & 30.21               \\
\textbf{SkipNet}                                     & 93.18            & 25.69               & 55.39            & 33.86               \\ \bottomrule
\end{tabular}
\end{table}
